Detecting New Planets in Transiting Systems

I present an initial investigation into a new planet detection technique that uses the transit timing of a known, transiting planet. The transits of a solitary planet orbiting a star occur at equally spaced intervals in time. If a second planet is present, dynamical interactions within the system will cause the time interval between transits to vary. These transit time variations can be used to infer the orbital elements of the unseen, perturbing planet. I show analytic expressions for the amplitude of the transit time variations in several limiting cases. Under certain conditions the transit time variations can be comparable to the period of the transiting planet. I also present the application of this planet detection technique to existing transit observations of the TrES-1 and HD209458 systems. While no convincing evidence for a second planet in either system was found from those data, I constrain the mass that a perturbing planet could have as a function of the semi-major axis ratio of the two planets and the eccentricity of the perturbing planet. Near low-order, mean-motion resonances (within about 1% fractional deviation), I find that a secondary planet must generally have a mass comparable to or less than the mass of the Earth--showing that these data are the first to have sensitivity to sub Earth-mass planets orbiting main sequence stars. These results show that TTV will be an important tool in the detection and characterization of extrasolar planetary systems.

==> 4chapter.tex <==
% results with simulated data stuff taken from aspen prep and annealing/paper

In this chapter I present the results of a preliminary study that addresses the possibility of determining the orbital elements of the perturbing planet by analyzing the transits of the known planet.  For this study I randomly generated several sets of orbital elements for a three-body system and used those systems to create sets of transit times.  I added noise of varying power to each of the sets of transit times.  Most of the analyses had noise whose RMS amplitude was equal to 10\% of the RMS signal amplitude.  This study focused on perturbing planets that are on orbits that are larger than the transiting planet and to planetary systems whose orbits are coplanar and edge-on.

\section{Software}

In effort to identify the orbital elements of an unknown perturbing planet from a given list of simulated transit times I integrate the equations of motion for a candidate three-body system using the Burlisch-Stoer integration algorithm.  When the transiting planet crosses the line of sight, the transit time is identified and tabulated.  These candidate transit times are compared to those of the simulated data and the quality of the fit of the orbital elements of the candidate system with those of the actual (simulated) system is characterized by the \cs\ statistic.

To locate the set of orbital elements that gives the minimum \cs, I sequentially employ a random and then a direct minimization algorithm.  For the random portion I generate many sets of orbital elements and record the \cs\ for each.  All parameters are drawn from a uniform distribution, except for the eccentricity and mass which are logarithmically uniform; between $10^{-3.4}$ and $1.0$ for the eccentricity and between $10^{-6}$ and $10^{-2.3}$ for the ratio of the planet to stellar mass.  I chose the logarithmic distribution so as to not assume a mass scale \textit{a priori}--our limits corresponding approximately to masses too small to be seen and too large to have not been seen.  This approach agrees with the empirical distribution of masses determined by \cite{tabac02}.  The logarithmic distribution was chosen for eccentricity because tidal circularization and orbital stability constraints favor small eccentricities ($\lesssim 0.1$).

I tabulate the two systems with the lowest \cs\ as starting points for the direct minimization algorithm.  Experiments with simulated data showed no significant improvement in the final \cs\ when more than two solutions were retained.  I assume, following the random minimization, that at least one set of orbital elements is near the global minimum of the \cs.  That is, the nearest local minimum is the global minimum and that the local gradient points toward that minimum.  From these points we use a direct minimization algorithm to locate the bottom of the global minimum.

The software is easily modified to find either an overall global minimum or to systematically step through any set of orbital elements, minimizing at each point over the remaining parameters.  Generally, I step through the semimajor axis ratio parameter though I have used other orbital elements for comparison purposes.  These analyses assume that the orbital elements of the transiting planet are known.

\section{Random Sample\label{randomsample}}

In effort to quantify the efficiency with which the TTV approach can determine the orbital elements of a peturbing planet I randomly generated the orbital elements for 150 coplanar planetary systems.  The semi-major axis ratio of the two planets was constrained to lie between 1.3 and 3.8---roughly between the $3:2$ and the $15:2$ mean-motion, orbital resonances.  For each of these systems I produce a table of 55 consecutive transit times.

I added noise to each of these data sets by first subtracting the best-fit line from the data and then adding Gaussian, white noise to each transit time where the standard deviation of the noise is equal to 10\% of the standard deviation of the original timing residuals.  I chose this approach for for this initial study---as opposed to adding absolute noise (i.e. noise that is a specific fraction of the period of the transiting planet instead of a fraction of the signal amplitude)---because I am primarily interested in the limitations of the method itself, given transit data.  Plans for future studies which use absolute timing noise are discussed later.

To determine the orbital elements of the perturbing planets in each of these systems I first conducted a coarse, systematic step through the semimajor axis ratio.  At each fixed value of axis ratio, I minimize over the remaining four parameters.  For each system, the orbital elements that corresponded to the minimum $\chi^2$ were compared to the actual orbital elements of the system.  I consider a successful identification to be when an estimated orbital element was within 5\% of the actual; most successful searches were much better.  Table \ref{searchresults} gives the number of successful identifications of the orbital elements as a function of this coarse, systematic search.

\begin{table}\label{searchresults}
\begin{center}
\caption{Overview of the results for the coarse search of 150 systems with 10\% timing noise.  A correct find indicates that the results of the search were within 5\% of the correct value.  For this study I did not treat the mass in the same manner as the other parameters.  Instead, I used it to linearly scale the amplitude of the timing deviations to match the data after I subtracted a linear fit from the transit times under consideration.  In all the studies after those in this section I did treat the mass in the same manner as the other orbital elements.
}
\vskip0.1in
\begin{tabular}{|c|c|} \hline
Find     & Number Correct \\ \hline \hline
$a$      & 108    \\ \hline
$e$      & 97     \\ \hline
$\varpi$ & 93     \\ \hline
$\tau$   & 17     \\ \hline
$m$      & 70     \\ \hline
\end{tabular}
\end{center}
\end{table}

For comparison purposes, I conducted similar searches for a subset of 30 systems where I stepped through parameters other than the semimajor axis ratio; namely the eccentricity, longitude of pericenter, and time of pericenter passage of the perturbing planet.  Table \ref{detailedresults} shows the number of correctly identified orbital elements for these searches.

\begin{table}\label{detailedresults}
\begin{center}
\caption{This table gives an overview of the different minimization approaches for a subset of 30 systems from the 150 randomly generated systems.  I list the number of successful finds, out of 30, for a particular parameter (shown in the row heading) depending upon the parameter that I systematically searched (shown in the column heading).  %Because these systems had a logarithmic distribution in eccentricity (between $10^{-3}$ and 1), there may be a bias away from the eccentricity search since the increments were linear and also some degeneracies between $\varpi$ and $\tau$.
}
\vskip0.1in
\begin{tabular}{|c|c|c|c|c|} \hline
Fit To & Step $a$ & Step $e$ & Step $\varpi$ & Step $\tau$ \\ \hline \hline
$a$      & 19 & 12 & 22 & 16 \\ \hline
$e$      & 16 & 13 & 19 & 17 \\ \hline
$\varpi$ & 18 & 17 & 14 & 18 \\ \hline
$\tau$   & 4  & 2  & 7  & 4  \\ \hline
\end{tabular}
\end{center}
\end{table}

I present here three of the randomly generated systems where the orbital elements were correctly identified to show, in more detail, the structure of the \cs\ near the minimum as well as the results of the fitting.  Table \ref{foundsystems} shows the actual and best-fitting parameters for these three systems and Figres \ref{sys1pic}, \ref{sys2pic}. and \ref{sys3pic} show plots of the \cs\ near the corresponding solutions.

\begin{table}\label{foundsystems}
\begin{center}
\caption{The results of the fit to systems 1, 2, and 3.  The \cs\ values are the lowest value for a quadratic fit to the minimum that is obtained from the coarse search through semimajor axis ratio.  Figures \ref{sys2pic}, and \ref{sys3pic} show the \cs\ at each value of semimajor axis ratio that was used for both the course seach and a refined search near the minimum of the coarse search.  Figure \ref{sys1pic} shows a contour plot of the \cs\ near the minimum in the $a$/$e$ plane where the remaining parameters are marginalized at each point.}
\vskip0.1in
\begin{tabular}{|c|c|c|c|c|c|c|} \hline
Parameter & \multicolumn{2}{c|}{System 1} & \multicolumn{2}{c|}{System 2} & \multicolumn{2}{c|}{System 3} \\ \hline
& Actual & Best-fit & Actual & Best-fit & Actual & Best-fit \\ \hline \hline
$a_2/a_1$       & 2.861 & 2.861 & 3.206 & 3.205 & 2.008 & 2.005 \\ \hline
$e_1$           & 0.007 & -     & 0.008 & -     & 0.027 & -     \\ \hline
$e_2$           & 0.014 & 0.015 & 0.014 & 0.013 & 0.001 & 0.002 \\ \hline
$\varpi_1/2\pi$ & 0.600 & -     & 0.477 & -     & 0.794 & -     \\ \hline
$\varpi_2/2\pi$ & 0.950 & 0.928 & 0.472 & 0.501 & 0.212 & 0.215 \\ \hline
$\tau_1/2\pi$   & 0.587 & -     & 0.717 & -     & 0.730 & -     \\ \hline
$\tau_2/2\pi$   & 0.147 & 0.839 & 0.850 & 0.014 & 0.186 & 0.456 \\ \hline
$m_1/m_J$       & 1.000 & -     & 1.465 & -     & 0.059 & -     \\ \hline
$m_2/m_J$       & 0.800 & 0.814 & 0.061 & 0.063 & 1.539 & 1.485 \\ \hline
$\chi^2_{\nu}$  & \multicolumn{2}{c|}{0.67} & \multicolumn{2}{c|}{0.77} & \multicolumn{2}{c|}{2.17} \\ \hline
\end{tabular}
\end{center}
\end{table}

\begin{figure}\label{sys1pic}
\includegraphics[width=\fsize]{confidence}
\caption{System 1: 1-$\sigma$, 2-$\sigma$, and 3-$\sigma$ confidence intervals for the results of a minimization for a randomly generated, coplanar system plotted in the $e-a$ plane (eccentricity on the $x$-axis and semi-major axis on the $y$-axis).  The white dot corresponds to the actual values of the system.  This minimization routine steps through $a$ and $e$ and marginalizes over the remaining parameters ($\varpi,\ \tau,\ m$).  The marginalization at each point occurs in two phases, a random search using simulated annealing followed by a direct search using a downhill-simplex (amoeba) algorithm.  55 transits are used to perform the minimization and the timing of each transit had 10\% timing noise added to it (Gaussian, white noise with a standard deviation equal to 10\% of the standard deviation of the timing residuals).  The minimum reduced $\chi^2$ was 0.67.  The results of this minimization is given in table 1, note that both the eccentricity and the semi-major axis were held fixed so the minimum may actually be displaced.}
\end{figure}

\begin{figure}\label{sys2pic}
\includegraphics[width=\fsize]{thegood1}
\includegraphics[width=\fsize]{thegood2}
\caption{System 2: (Upper Image) Reduced $\chi^2$ as a function of semi-major axis ratio, the orbital elements of the transiting planet are assumed to be known and the remaining parameters are marginalized at each step.  This systems was chosen from a randomly generated set of 30 planets.  This coarse search correctly located the axis ratios of 19 of 30 systems to within 0.05 (18 to within 0.01).  (Lower Image) Reduced $\chi^2$ for the same system with a refined search near the minimum of the \cs.  The results of these searches are given in table 1.}
\end{figure}

\begin{figure}\label{sys3pic}
\includegraphics[width=\fsize]{thegood3}
\includegraphics[width=\fsize]{thegood4}
\caption{System 3: (Upper Image) Reduced $\chi^2$ as a function of semi-major axis ratio, the orbital elements of the transiting planet are assumed to be known and the remaining parameters are marginalized at each step.  This system was also chosen from the randomly generated set of 30 planetary systems.  (Lower Image) Reduced $\chi^2$ for the same system with a refined search near the minimum of each system.  The results of these searches are given in table 1.}
\end{figure}

%\begin{figure}
%\includegraphics[width=\fsize]{earth12}
%\includegraphics[width=\fsize]{earth17}
%\caption{Results of randomly generated planets perturbing HD209458b.  When the planets were selected between 8 and 1/3 of an Earth mass at least 14 of 30 were found found using the coarse search in semi-major axis ratio (the computer is still finishing the analysis of several systems).  When the planets were selected between 2 Jupiter masses and 2/3 of an Earth mass, 20 of 30 were found with the coarse search through the axis ratio.}
%\end{figure}

The results given in Tables \ref{searchresults} and \ref{detailedresults} indicate that, at least, a significant fraction the orbital elements can be identified from the transit times.  Additional studies may provide more efficient means to determine these elements.  I discuss one possibility next, in section \ref{fouriersearch}.  Regardless, the TTV technique appears to be capable of identifying the orbital elements of many planetary systems.

\section{Fourier Analysis of TTV Signal\label{fouriersearch}}

Since the TTV signal is typically periodic, it may be possible to use a discrete Fourier transform (FT) of the timing deviations to identify several of the orbital elements of the system---the ultimate goal of the technique.  An analysis conducted with a Fourier representation of the data may even be more appropriate for finding the semimajor axis ratio of the system than analyzing the data in the time basis because the orbit of the periodic nature of the systems involved.  Other orbital elements may also be determined with the Fourier representation, though such a development is left for elsewhere.

Here, I briefly introduce a method to determine the semimajor axis ratio of the planetary system using a Fourier transform of the timing deviations.  The value of this technique is that it could reduce the parameter space by one parameter entirely or, at least, provide several individual values about which a more complete search can be conducted.  This technique may also give an independent confirmation of an estimate for the semimajor axis ratio parameter that is obtained by another means.

\subsection{Fourier Representation}

Consider figures \ref{fourres} and \ref{fournonres}.  Figure \ref{fourres} shows the timing residuals of the transits of a planet where the perturber is near a mean-motion orbital resonance (the 2:1 resonance in this case).  The second image in this picture shows the FT of those residuals.  The symmetry in the Fourier transform is due to the fact that the timing information is encapsulated in both the amplitude and the phase of the Fourier components so that only the Fourier components up to the Nyquist frequency (half-way across the graph) contain unique information.  For this case the Fourier component that corresponds to the 2:1 resonant forcing term has the largest amplitude.  By comparison, figure \ref{fournonres} is for a system that is not near an orbital resonance and has several large peaks in the amplitudes of the Fourier components.

\begin{figure}
\includegraphics[width=\fsize]{deltat15}
\includegraphics[width=\fsize]{fourier15}
\caption{Timing residuals (upper panel) with Fourier transform of those residuals (lower panel) for a planetary system that is near a mean-motion resonance.}
\label{fourres}
\end{figure}

\begin{figure}
\includegraphics[width=\fsize]{deltat56}
\includegraphics[width=\fsize]{fourier56}
\caption{Timing residuals (upper panel) with Fourier transform of those residuals (lower panel) for a planetary system that is not near a mean-motion resonance.}
\label{fournonres}
\end{figure}

In order to determine whether or not the relative spacing between the peaks in the FT was interesting, I generated a set of planetary systems where both planets had zero eccentricity, equal mass, equal time of pericenter passage, and with various, equally spaced semimajor axis ratios with the perturber being exterior to the transiting planet.  For each system I tabulated the variations in transit time and then took the FT of the timing residuals.  I then calculated the time intervals that correspond to the largest peaks (up to five) of the FT.

From these results I generated a scatter plot of the values of the five time intervals as a function of the semimajor axis ratio and obtained figure \ref{thing1}.  Each of the visible peaks corresponds to a particular mean-motion resonance---the shape of which is given later.  One of the remaining structures is a diagonal line that corresponds to the period of the perturbing planet in units of the period of the transiting planet.  This diagonal line is particularly interesting because it is invertable and can, therefore, be used to uniquely identify the period of the perturbing planet.

\begin{figure}
\includegraphics[width=\fsize]{periodsnodots}
\caption{This picture shows the periods that correspond to the five largest peaks in the Fourier transform of the timing residuals for a transiting planet where both planets are on initially circular orbits as a function of the ratio of the semimajor axes of the planets.  The period that corresponds to the highest peak is in red, the second highest is in yellow, then green, blue, and purple.\label{thing1}}
\end{figure}

The overall structure of this graph is virtually independent of the orbital elements of the system.  For example, another set of systems, with identical values of the semimajor axis ratio but with the remaining orbital elements being randomly generated results in Figure \ref{thing2}.  The primary difference between Figures \ref{thing1} and \ref{thing2} is that the relative heights of the various peaks in the FT; the peaks themselves remain in the same locations.

\begin{figure}
\includegraphics[width=\fsize]{periodsrandom}
\caption{Similar to Figure \ref{thing1}, this shows the periods that correspond to the five largest peaks in the Fourier transform of the timing residuals as a function of the semimajor axis ratio of the two planets.  Here the orbital elements of the systems at each axis ratio are randomly selected.  Red corresponds to the highest peak, then yellow, green, blue, and purple.\label{thing2}}
\end{figure}

The shape of the peaks that are visible in these two plots can be derived from the corresponding mean motion resonance.  For the $i$:$j$ resonance, where $i$ and $j$ are integers and where $iP_{\text{trans}}=jP_{\text{pert}}$ corresponds to exact resonance, the period that describes the shape of the structures in Figures \ref{thing1} and \ref{thing2} is given by
\begin{equation}\label{lines}
\frac{P_{\text{peak}}}{P_{\text{trans}}} = \frac{P_{\text{pert}}}{iP_{\text{trans}}-jP_{\text{pert}}}.
\end{equation}
This shows that the period of the Fourier component that appears on a given peak approaches infinity as the system approaches the resonance and falls away as the distance from that resonance increases.  Figure \ref{thing3} superposes several curves of equation (\ref{lines}), that correspond to different resonances, onto Figure \ref{thing1}.

\begin{figure}
\includegraphics[width=\fsize]{periodswiththeo}
\caption{This figure has the plot from Figure \ref{thing1} with several curves of equation \ref{lines} superposed.  Also shown are the two diagonal lines that correspond to the period of the perturbing planet (upper diagonal line) and half the period of the perturbing planet (lower diagonal line).\label{thing3}}
\end{figure}

The value of this development is that the Fourier information can be used as a fingerprint to identify the period of the perturbing planet directly from the transform of the timing residuals.  Starting with the FT of a given set of timing residuals we plot the periods that are associated with the peaks in the amplitude of the FT.  We then assume that one of the peaks is precisely the period of the perturbing planet and compare the remaining peaks with the set of periods that result from equation (\ref{lines}).  For example, in Figure \ref{thing4} I show the periods that correspond to the peaks in the FT of the systems shown in Figures \ref{fourres} and \ref{fournonres} superposed upon Figure \ref{thing1}.

\begin{figure}
\includegraphics[width=\fsize]{periodswithdots}
\caption{This figure has the plot from Figure \ref{thing1} with the periods that correspond to the highest peaks in the Fourier transform---shown in black---of the resonant system whose transit times are shown in Figure \ref{fourres} (on the left) and the nonresonant system whose transit times are shown in Figure \ref{fournonres}.\label{thing4}}
\end{figure}

\subsection{Implementation}

Several tasks remain to be done before this technique to determine the semimajor axis ratio of the planetary system can be implemented in a robust and automated manner.  The largest impedement is that I have not found an appropriate statistical test to estimate the proper fit of the Fourier peaks to equation (\ref{lines}).  I initially tried several systems ``by eye'' and found that I could correctly identify approximately 90\% of the systems---though no noise had been added to the transit timings.  Most of the remaining systems had several possibilities that looked as though they fit equally well.

The difficulty lies in the fact that there are infinitely many resonances against which the data could be tested; but they are not equally important.  One could probably find a perfect fit to the Fourier peaks if he were allowed to include the effects of resonances such as the 6:3 resonance---which corresponds to the 2:1 resonance but still provides an independent curve from equation (\ref{lines}) (this can be seen in Figure \ref{thing1})---or the 200:101 resonance which is also near the 2:1 resonance but which is intuitively less important.  There is no clear method to determine which resonances should be weighted more heavily than others.  One potentially fruitful method would be to weight each higher order resonance (where the order is defined by $|i-j|$) by the maximum, average, or product of the eccentricities of the planets.  Thus, for low-eccentricity systems the importance of the high-order resonances would be severely limited; while for highly eccentric systems they would be more important.

Another challenge is that there are not always multiple peaks that can be identified in the FT---see the Figures \ref{fourres} and \ref{fournonres}.  Any noise that is added to the data will tend to wash out one or more of the peaks regardless of its importance to determining the semimajor axis ratio parameter.  For example, in the resonant system of Figure \ref{fourres}, the second largest peak corresponds to the (unique) period of the perturbing planet.  This peak is significantly smaller than the peak that corresponds to the 2:1 resonance; but without it there is no way to identify that the resonance is indeed 2:1---any resonance would be a candidate.  I have yet to determine an appropriate way to handle this issue and the one discussed in the preceeding paragraph.  Until such time as these problems have been solved the value of this Fourier technique is uncertain.  It does, however, illustrate the potential that the technique posseses.

\section{Effects of Noise and Coverage Gaps\label{noisesec}}

We now turn our discussion to the effects that lie largely beyond the control of the Earth-bound and mortal observer.  That is, the effects of noise, gaps between observed transits, and the number of observations that can be reasonably obtained for a system.  This discussion will remain somewhat cursory as many of the details of these effects await future developments (see section \ref{plans} for planned studies).

\subsection{Timing Noise}

I have not conducted a formal or analytical investigation of the effects of timing noise---that is, uncertainty in the time of transit.  However, I discuss some effects that I have seen in my numerical work to this point.  While noise clearly affects one's ability to determine the orbital elements in question, the degree to which timing noise mars the signal is a function of both the true system parameters (e.g. proximity to resonance) and the number of observations.

If the timing variations are periodic, which is typically the case, then you can overcome the effects of timing noise by simply increasing the number of observations.  However, this approach is not always feasable as the period of the variations can be quite large depending upon the proximity to resonance in the system.  As you approach resonance, the period of the variations grows large.  Fortunately, a competing effect is that the signal is significantly larger as you approach a resonance.  So, provided that the observations are taken over a baseline that is large enough to see the turning point in the timing variations, a resonant system can be seen more readily for a given amount of timing uncertainty than can a nonresonant system.

To illustrate this, consider the FT of the timing variations shown in Figures \ref{fourres} and \ref{fournonres}.  The amplitude of the resonant Fourier component is significantly larger than the overall amplitude of the FT of the timing residuals.  Moreover, it is much larger than the amplitude of the Fourier components of the nonresonant system.  This fact follows from Parseval's relation which states that the sum of the squares of the Fourier components is proportional to the sum of the squares of the timing deviations.  Since the resonant variations are larger than the nonresonant ones, its FT should also be larger.

If (Gaussian, white) timing noise is added to the timing residuals it would be equivalent to adding a equal signal at every frequency in the FT.  In a resonant system, where most of the signal is concentrated in one frequency channel, it would take a significant amount of noise being added to the timings in order to ``raise the floor'' in Fourier space up to the same amplitude as the resonant component.  Indeed, it would take timing noise with an amplitude that is significantly larger than the signal amplitude (in the time domain) in order to wash the signal out.  The same is not true for a nonresonant system where the signal is distributed among several Fourier components.  Such signals are washed out more readily by added noise because the different peaks in the FT are not as prominent as that of the single peak in the resonant system. Thus, even though the timing variations in resonant systems have a longer period, the fact that the signal is concentrated into only a few Fourier components makes them less susceptible to the effects of timing noise.

%\begin{figure}
%\includegraphics[width=0.45\textwidth]{noise028}
%\includegraphics[width=0.45\textwidth]{noise092}
%\vskip0.1in
%\includegraphics[width=0.45\textwidth]{noise303}
%\includegraphics[width=0.45\textwidth]{noise999}
%\caption{Reduced $\chi^2$ for System 1 with Gaussian, white noise added where the standard deviation of the noise is equal to 30\% (top left), 92\% (top right), 300\% (bottom left), and 1000\% (bottom right) of the standard deviation of the timing residuals as a function of the semi-major axis ratio of the system.  This analysis uses 55 data points.}
%\end{figure}

\subsection{Coverage Gaps}

The continuous monitoring of exoplanetary systems requires space-based platforms that are dedicated to these observations (e.g. \textit{Kepler}).  So, gaps in the transit observations will generally occur.  I do not know the extent to which coverage gaps will affect ones ability to determine the orbital elements of a planetary systems using TTV.  It is likely that the Fourier technique presented earlier will suffer somewhat simply because, while a frequency domain representation that involves sparse data, such as a periodogram, may provide the same resolution as an equal number of contiguous data that uses this Fourier technique, the coverage gaps necessarily degrade the resolution that can be obtained with data taken over an equal observational baseline---the real timeline of a scientific program.  Also, coverage gaps, if they are periodic, will certainly cause any periodicities in the data to mix with the observations in a potentially nontrivial manner.  They are also likely to produce spurious solutions as discussed in the next chapter (see section \ref{search}).

Otherwise, as a part of the study of the TrES-1 system, that I present in the next chapter, I removed transits from some of the (correctly identified) systems that I analyzed in section \ref{randomsample} such that the gaps in coverage matched those of the TrES-1 data.  I then re-analyzed those systems to see if I could recover their orbital elements.  The result was that I was indeed able to recover the same results without fail.  The only difference was that additional relative minima appeared in the \cs , that the \cs\ curve, as a function of semimajor axis ratio was more noisy, and that the precision with which the elements could be identified was degraded.

\section{Future Studies\label{plans}}

As I continue to investigate the issue of determining the orbital elements of a planetary system via TTV, I will address several issues that either prompted or have been raised by this preliminary study.  In particular, I will conduct a similar investigation to that presented at the beginning of this chapter (section \ref{randomsample}) with randomly generated systems; this time with absolute timing noise added (e.g. noise that is $10^{-5}P_{\text{trans}}$).  In conjunction with this study I will investigate in more depth the effect that timing noise has on a TTV analysis.

Also, I plan to probe the effects of coverage gaps in more detail.  This effort should provide an acceptable attempt to maximize the number of systems that can be found with limited resources.  Finally, I will address the effects of mutually inclined orbits.  The primary impediment to these plans is the existing analysis software.  For the near future I will upgrade this software to make it more flexible and to improve the approach that I take for the analysis---in short, I need to take a work of art and turn it into an equally beautiful engineering masterpiece.

